Non-asymptotic Convergence Analysis of Two Time-scale (Natural) Actor-Critic Algorithms

As an important type of reinforcement learning algorithms, actor-critic (AC) and natural actor-critic (NAC) algorithms are often executed in two ways for finding optimal policies. In the first nested-loop design, actor's one update of policy is followed by an entire loop of critic's updates of the value function, and the finite-sample analysis of such AC and NAC algorithms have been recently well established. The second two time-scale design, in which actor and critic update simultaneously but with different learning rates, has much fewer tuning parameters than the nested-loop design and is hence substantially easier to implement. Although two time-scale AC and NAC have been shown to converge in the literature, the finite-sample convergence rate has not been established. In this paper, we provide the first such non-asymptotic convergence rate for two time-scale AC and NAC under Markovian sampling and with actor having general policy class approximation. We show that two time-scale AC requires the overall sample complexity at the order of $\mathcal{O}(\epsilon^{-2.5}\log^3(\epsilon^{-1}))$ to attain an $\epsilon$-accurate stationary point, and two time-scale NAC requires the overall sample complexity at the order of $\mathcal{O}(\epsilon^{-4}\log^2(\epsilon^{-1}))$ to attain an $\epsilon$-accurate global optimal point. We develop novel techniques for bounding the bias error of the actor due to dynamically changing Markovian sampling and for analyzing the convergence rate of the linear critic with dynamically changing base functions and transition kernel.

==> ttsNAC.tex <==
\section{Two Time-scale AC and NAC}\label{sc: tts_ac}
We now introduce the AC and NAC algorithms studied in this paper. As explained in Section \ref{sc: MDP}, the transition kernel adopts $\widetilde{\mathsf{P}}(\cdot |s,a)=\gamma\mathsf{P}(\cdot |s,a)+(1-\gamma)\xi(\cdot)$. 

In this paper, we study the AC algorithm that adopts the design proposed in \cite{konda2002actor} (as detailed in Algorithm \ref{algorithm_ttsac}). The algorithm updates in a two time-scale fashion. Namely, actor and critic update simultaneously but with different stepsizes: actor updates at a slow times scale to optimize the policy $\pi_w$, and critic updates at a fast time scale to estimate the advantage function $A_\theta(s,a)$. More specifically, at step $t$, actor updates the parameter $w_t$ of policy $\pi_w$ using a stochastic version of the policy gradient in \cref{pg_gradient} given by
\begin{flalign*}
w_{t+1}=w_t+\alpha_t\widetilde{\nabla}J(w_t,\theta_t).
\end{flalign*}
where $\widetilde{\nabla}J(w_t,\theta_t) = A_{\theta_t}(s_t,a_t)\phi_{w_t}(s_t,a_t)$ and $\alpha_t>0$ is the stepsize. Note that if $\theta_t$ is a good estimate of the minimum norm solution of \cref{eq: solu1}, then $\widetilde{\nabla}J(w_t,\theta_t)$ is a good stochastic approximation of $\nabla J(w_t)$ if we let $\phi(s,a)=\phi_{w_t}(s,a)$. This is guaranteed by critic's update at fast time-scale as we introduce below.

Critic's update follows the linear SA algorithm with dynamically changing base function and transition kernel, which adopts $\text{Q-Sampling}(s,a,\pi)$ (see \Cref{algorithm_qsample}) proposed by \cite{zhang2019global} with an unbiased estimator of the state-action value function $Q_\pi(s,a)$ as the output.
%Now we consider the update of the critic. 
Critic's update of the parameter $\theta$ is to find the solution for \cref{eq: solu1}. Clearly, the objective function $L_w(\theta)$ is quadratic, and can be minimized efficiently using the stochastic gradient descent (SGD) algorithm. We first give the full gradient as follows:
\begin{flalign*}
-\nabla_\theta L_w(\theta)&=\mE_{\nu_{\pi_{w}}}[-\phi_w(s,a)\phi_w(s,a)^\top \theta]+\mE_{\nu_{\pi_{w}}}[A_{\pi_{w}}(s,a)\phi_w(s,a)  ].
\end{flalign*}
To estimate the gradient $-\nabla_\theta L_w(\theta)$, note that
\begin{flalign*}
\mE_{(s,a)\sim\nu_{\pi_{w}}}&[A_{\pi_{w}}(s,a)\phi_w(s,a)  ] \\
&= \mE_{(s,a)\sim\nu_{\pi_{w}}}[Q_{\pi_{w}}(s,a)\phi_w(s,a)  ] - \mE_{(s,a^\prime)\sim\nu_{\pi_{w}}}[V_{\pi_w}(s)\phi_w(s,a^\prime)  ]\\
&=\mE_{(s,a)\sim\nu_{\pi_{w}}}[Q_{\pi_{w}}(s,a)\phi_w(s,a)  ] - \mE_{(s,a^\prime)\sim\nu_{\pi_{w}}}\big[\mE[Q_{\pi_w}(s,a)|s,a^\prime]\phi_w(s,a^\prime)  \big].
\end{flalign*}
Thus, at time $t$, with parameters $w_t$ and $\theta_t$, we can sample the MDP to estimate the gradient $-\nabla_\theta L_{w_t}(\theta_t)$ as
\begin{flalign*}
\hat{g}_{i}(\theta_t)=(-\phi_{w_t}(s_i,a_i)^\top\theta_t+\widehat{Q}_{\pi_{w_t}}(s_i,a_i))\phi_{w_t}(s_i,a_i)-\widehat{Q}_{\pi_{w_t}}(s_i,a_i)\phi_{w_t}(s_i,a^\prime_i) - \lambda\theta_t,
\end{flalign*} 
where $a_i$ and $a^\prime_i$ are sampled independently from the policy $\pi_{w_t}(\cdot|s_i)$, and the regularization term $\lambda \theta_t$ is added here to prevent the divergence of critic's iteration (namely, to prevent the matrix of the corresponding ordinary differential equation (ODE) of linear SA from being singular). Such a stability condition is typically required for the analysis of linear SA in the literature \cite{dalal2018finite,bhandari2018finite}. We further note that the base function $\phi_{w_t}$ of critic, which is also the score function of policy $\pi_{w_t}$, changes as actor updates, so that the compatible condition \cite{sutton2000policy,konda1999actor} can always be satisfied. 

Alternatively, natural actor-critic (NAC) (see Algorithm \ref{algorithm_ttsac}) \cite{bhatnagar2009natural,agarwal2019optimality} utilizes natural gradient ascent  \cite{amari1998natural,kakade2002natural}, which guarantees that the policy update is invariant to the parameterization of the policy. Similarly to AC, NAC here also adopts the two time-scale update with actor in the slow time-scale and critic at fast time-scale. At each step $t$, ideally actor's update should be given by
\begin{flalign}
w_{t+1}=w_t+\alpha_t F(w_t)^\dagger\nabla J(w_t),\label{eq: npg}
\end{flalign}
where $F(w_t)$ is the Fisher information matrix defined as $F(w_t)\coloneqq\mE_{\nu_{\pi_{w_t}}}\big[ \phi_{w_t}(s,a) \phi_{w_t}(s,a)^\top \big]$, and $F(w_t)^\dagger$ represents the pseudoinverse of $F(w_t)$. However, it is intractable to perform the update in \cref{eq: npg} exactly as the visitation distribution $\nu_{\pi_{w_t}}$ is usually unknown. It can be checked easily that the minimum norm solution of the problem in \cref{eq: solu1} satisfies $\theta^\dagger_{w_t}=F(w_t)^\dagger\nabla J(w_t)$. Thus, a practical way to perform the NAC is to let critic solve \cref{eq: solu1} approximately such that $\theta_t\approx \theta^\dagger_{w_t}$ \cite{agarwal2019optimality}, and then the actor updates the parameter of the policy as
\begin{flalign*}
w_{t+1}=w_t+\alpha_t \theta_t.
\end{flalign*}


We set the two stepsizes as $\alpha_t=\Theta(1/(t+1)^\sigma)$ and $\beta_t=\Theta(1/(t+1)^\nu)$, with $0<\nu<\sigma\leq 1$. Let
$\mcpi_{R_\theta}$ denote the projection operator onto a norm ball with the radius satisfying $\max_{w\in \mR^d}\{ \theta^*_w \}\leq R_\theta\leq C_b/\lambda_P\leq C_b/\lambda$. Here we use the projection in critic's update to prevent actor from taking a large step in a "wrong" direction, which has been commonly adopted in \cite{konda2000actor,konda2002actor,wang2019neural}. We define the output distribution at time $t$ as $P_{T}(i)=\text{Prob}(x=i)=\frac{\alpha_i}{\sum_{i=0}^{T-1}\alpha_i}$. Since $\alpha_t/\beta_t\rightarrow0$ as $t\rightarrow\infty$, $w_t$ is almost static with respect to $\theta_t$ asymptotically. If we treat $w_t$ as a fixed vector, then the critic is expected to track the fix point $\theta^*_{w_t}$ of the corresponding ODE. Thus, if $t$ is sufficiently large, we expect $\theta_t$ to be close to $\theta^*_{w_t}$. Note that Algorithm \ref{algorithm_ttsac} does not require the accessibility of the visitation distribution, as all state-action pairs are sampled sequentially by policy $\pi_{w_t}$ that changes dynamically as $w_t$ is updated.

\begin{algorithm}[tb]
	\caption{Two Time-scale AC and NAC}
	\label{algorithm_ttsac}
	\begin{algorithmic}
		\STATE {\bfseries Input:} Parameterized policy $\pi_w$, actor stepsize $\alpha_t$, critic stepsize $\beta_t$, regularization constant $\lambda$
		\STATE {\bfseries Initialize:} actor parameter $w_0$, critic parameter $\theta_0$
		\FOR{$t=0,\cdots,T-1$}
		\STATE $s_t\sim \widetilde{\mathsf{P}}(\cdot |s_{t-1},a_{t-1})$
		\STATE Sample $a_t$ and $a^\prime_t$ independently from $\pi_{w_t}(\cdot|s_t)$
		\STATE $\widehat{Q}(s_t,a_t)=\text{Q-Sampling}(s_t,a_t,\pi_{w_t})$
%		\STATE $\phi_{w_t}(s_t,a_t)=\nabla_w\log\pi_{w_t}(a_t|s_t)$
%		\STATE $\phi_{w_t}(s_t,a^\prime_t)=\nabla_w\log\pi_{w_t}(a^\prime_t|s_t)$
		\STATE $g_t(\theta_t)=(-\phi_{w_t}(s_t,a_t)^\top\theta_t+\widehat{Q}(s_t,a_t))\phi_{w_t}(s_t,a_t)$
		$-\widehat{Q}(s_t,a_t)\phi_{w_t}(s_t,a^\prime_t) - \lambda\theta_t$
		\STATE  
		\STATE  \textit{\textbf{Critic Update: }}$\theta_{t+1}=\mcpi_{R_\theta}(\theta_t+\beta_t g_t(\theta_t))$
		\STATE
		\STATE \textit{\textbf{Option I: Actor update in AC}}
		\STATE $w_{t+1}=w_t+\alpha_t [\phi_{w_t}(s_t,a_t)^\top\theta_{t}]\phi_{w_t}(s_t,a_t)$
		\STATE
		\STATE \textit{\textbf{Option II: Actor update in NAC}}
		\STATE $w_{t+1}=w_t+\alpha_t \theta_{t}$
		\ENDFOR
		\STATE {\bfseries Output:} $w_{\hat{T}}$ with $\hat{T}$ chosen from distribution $P_{T}$
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[tb]
	\caption{$\text{Q-Sampling}(s,a,\pi)$}
	\label{algorithm_qsample}
	\begin{algorithmic}
		%\STATE {\bfseries Input:} state $s$, action $a$ and policy $\pi$
		\STATE {\bfseries Initialize:} $\widehat{Q}_\pi(s,a)=0$, $s_0=s$ and $a_0=a$
		\STATE $T\sim \text{Geom}(1-\gamma^{1/2})$
		\FOR {$t=0,\cdots,T-1$}
		\STATE $s_{t+1}\sim \mathsf{P}(\cdot|s_t,a_t)$
		\STATE $\widehat{Q}_\pi(s,a)\leftarrow\widehat{Q}_\pi(s,a)+\gamma^{t/2}r(s_t,a_t,s_{t+1})$
		\STATE $a_{t+1}\sim \pi(\cdot|s_{t+1})$
		\ENDFOR
		\STATE {\bfseries Output:} $\widehat{Q}_\pi(s,a)$
	\end{algorithmic}
\end{algorithm}

\subsection{Technical Assumptions}
We take the following standard assumptions throughout the paper.
\begin{assumption}\label{ass1}
	For any $w,w^\prime\in R^d$ and any state-action pair $(s,a)\in \mcs\times\mca$, there exist positive constants $L_\phi$, $C_\phi$, and $C_\pi$ such that the following hold:
	\begin{enumerate}
		\item $\ltwo{\phi_w(s,a)-\phi_{w^\prime}(s,a)}\leq L_{\phi}\ltwo{w-w^\prime}$,
		\item $\ltwo{\phi_w(s,a)}\leq C_\phi$,
		\item $\lTV{\pi_w(\cdot|s)-\pi_{w^\prime}(\cdot|s)}\leq C_\pi\ltwo{w-w^\prime}$, where $\lTV{\cdot}$ denotes the total-variation norm.
	\end{enumerate}
\end{assumption}
The first two items in \Cref{ass1} assume that the score function $\phi_w$ is smooth and bounded, which have also been adopted in previous studies \cite{kumar2019sample,zhang2019global,agarwal2019optimality,konda2002actor,zou2019finite}. The first two items can be satisfied by many commonly used policy classes including some canonical policies such as Boltzman policy \cite{konda1999actor} and Gaussian policy \cite{doya2000reinforcement}. 
The third item in \Cref{ass1} holds for any smooth policy with bounded action space or Gaussian policy. For justification of the third item please refer to Lemma 1 in our last paper \cite{xu2019improved}.

\begin{assumption}[Ergodicity]\label{ass2}
	For any $w\in\mR^d$, consider the MDP with policy $\pi_w$ and transition kernel $\mathsf{P}(\cdot|s,a)$ or $\widetilde{\mathsf{P}}(\cdot|s,a)=\gamma \mathsf{P}(\cdot|s,a) + (1-\gamma)\eta(\cdot)$, where $\eta(\cdot)$ can either be $\xi(\cdot)$ or $\mathsf{P}(\cdot|\hat{s},\hat{a})$ for any given $(\hat{s},\hat{a})\in \mathcal{S}\times\mathcal{A}$. There exist constants $\kappa>0$ and $\rho\in(0,1)$ such that
	\begin{flalign*}
	\sup_{s\in\mcs}\lTV{\mP(s_t\in\cdot|s_0=s)-\chi_{\pi_w}}\leq \kappa\rho^t,\quad \forall t\geq 0,
	\end{flalign*}
	where $\chi_{\pi_w}$ is the stationary distribution of the corresponding MDP with transition kernel $\mathsf{P}(\cdot|s,a)$ or $\widetilde{\mathsf{P}}(\cdot|s,a)$ under policy $\pi_w$.
\end{assumption}
Assumption \ref{ass2} has also been adopted in the previous studies \cite{bhandari2018finite,xu2020reanalysis,zou2019finite}, which holds for any time-homogeneous Markov chain with finite state space or any uniformly ergodic Markov chain with general state space.

